Invertibility in Category Representations

Inverse categories are categories in which every morphism x has a unique pseudo-inverse y in the sense that xyx=x and yxy=y. Persistence modules from topological data analysis and similarly decomposable category representations factor through inverse categories. This paper gives a numerical condition, decidable when the indexing category is finite, characterizing when a representation of a small category factors through an inverse category.

==> notation.tex <==
\DeclareMathAlphabet{\callrsfs}{OT1}{pzc}{m}{it} 

\makeatletter
\newcommand{\dashover}[2][\mathop]{#1{\mathpalette\df@over{{\dashfill}{#2}}}}
\newcommand{\df@over}[2]{\df@@over#1#2}
\newcommand\df@@over[3]{%
  \vbox{
    \offinterlineskip
    \ialign{##\cr
      #2{#1}\cr
      \noalign{\kern1pt}
      $\m@th#1#3$\cr
    }
  }%
}
\newcommand{\dashfill}[1]{%
  \kern-.5pt
  \xleaders\hbox{\kern.5pt\vrule height.4pt width \dash@width{#1}\kern.5pt}\hfill
  \kern-.5pt
}
\newcommand{\dash@width}[1]{%
  \ifx#1\displaystyle
    2pt
  \else
    \ifx#1\textstyle
      1.5pt
    \else
      \ifx#1\scriptstyle
        1.25pt
      \else
        \ifx#1\scriptscriptstyle
          1pt
        \fi
      \fi
    \fi
  \fi
}
\makeatother

% general
\newcommand{\I}{\mathbb{I}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}

% formatting
\newcommand{\backspace}{\!\!\!\!\!\!\!}
\newcommand{\upsidedown}[1]{\reflectbox{\rotatebox[origin=c]{180}{#1}}}
\newcommand\circumscribe[1]{\stackMath\mathbin{\stackinset{c}{0ex}{c}{0ex}{#1}{\bigcirc}}}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}

% greek
\newcommand{\Tau}{\mathrm{T}}
\newcommand{\Iota}{\mathrm{I}}

% category theory
\newcommand{\catfont}[1]{\mathrm{\bf #1}}
\newcommand{\coequalizer}[5]{\xymatrix@C=6pc{#1\ar@<.7ex>[r]^{#4}\ar@<-.7ex>[r]_{#5} & #2\ar@{.>}[r] & #3}}
\newcommand{\LAN}[2]{\mathrm{LAN}_{#2}{#1}}
\newcommand{\forget}{\mathfrak{forget}}
\newcommand{\NFOLDGROUPS}[2]{\calligra{grp}^{#1}_{#2}}
\newcommand{\smallcat}[1]{\ifthenelse{1=#1}{X}{\ifthenelse{2=#1}{Y}{Z}}}
\newcommand{\smallgroupoid}[1]{\ifthenelse{1=#1}{\mathcal{G}}{\mathcal{H}}}
\newcommand{\modelcat}[1]{\ifthenelse{1=#1}{\mathscr{M}}{\ifthenelse{2=#1}{\mathscr{N}}{\mathscr{O}}}}
\newcommand{\cat}[1]{\ifthenelse{1=#1}{\mathscr{X}}{\ifthenelse{2=#1}{\mathscr{Y}}{\mathscr{Z}}}}
\newcommand{\groupoid}[1]{\ifthenelse{1=#1}{\mathscr{G}}{\ifthenelse{2=#1}{\mathscr{H}}{\mathscr{I}}}}
\newcommand{\shape}[1]{\ifthenelse{1=#1}{\bigcirc}{\ifthenelse{2=#1}{\pentagon}{\octagon}}}
\newcommand{\doublecat}[1]{\ifthenelse{1=#1}{\mathfrak{C}}{\ifthenelse{2=#1}{\mathfrak{D}}{\mathfrak{E}}}}
\newcommand{\doublefunctor}[1]{\ifthenelse{1=#1}{\mathfrak{F}}{\ifthenelse{2=#1}{\mathfrak{G}}{\mathfrak{H}}}}
\newcommand{\BASED}[1]{#1_{\star}}
\newcommand{\adjoint}{\mathfrak{adj}}
\newcommand{\Aut}{\mathop{Aut}}
\newcommand{\Hom}{\mathop{Hom}}
\newcommand{\la}{\leftarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\rras}{\rightrightarrows}
\newcommand{\partialra}{\rightharpoonup}
\newcommand{\xra}{\xrightarrow}
\newcommand{\xla}{\xleftarrow}
\newcommand{\xira}{\xhookrightarrow}
\newcommand{\lras}{\leftrightarrows}
\newcommand{\ira}{\hookrightarrow}
\newcommand{\colim}{\mathrm{colim}}
\newcommand{\holim}{\mathrm{holim}}
\newcommand{\hocolim}{\mathrm{hocolim}}
\newcommand{\id}{1}
\newcommand{\im}{{\mathop{im}}}
\newcommand{\counit}{\epsilon}
\newcommand{\unit}{\eta}
\newcommand{\free}{\calligra{free}}
\newcommand{\pullback}[1]{{#1}^*}
\newcommand{\pushforward}[1]{{#1}_*}
\newcommand{\cardinality}{\#}
\newcommand{\OP}[1]{#1^{\mathrm{op}}}
\newcommand{\WE}{\mathop{h}}
\newcommand{\DERIVED}{\mathscr{D}}
\newcommand{\PAIRS}[1]{(#1,#1)}
\newcommand{\CUBICAL}{c}
\newcommand{\MONOIDS}{\catfont{Mon}}
\newcommand{\RANKEDPOSETS}{\catfont{Pos}_{*}}
\newcommand{\VECTORSPACES}{\catfont{Vec}}
\newcommand{\SEMILATTICES}{\catfont{Sem}}
\newcommand{\SIMPLICIAL}{s}
\newcommand{\BI}[1]{#1 #1}
\newcommand{\GENERIC}{\mathscr{X}}
\newcommand{\SMALLGENERIC}{\mathcal{X}}
\newcommand{\PREORDEREDSETS}{\mathscr{Q}}
\newcommand{\SEMIMODULES}{\mathscr{M}}
\newcommand{\ALGEBRAS}{\mathscr{A}}
\newcommand{\CATS}{\catfont{Cat}}%{\calligra{Cat}}
\newcommand{\DOUBLECATS}{\calligra{Cat^{(2)}}}%{\calligra{Cat}}
\newcommand{\GROUPOIDS}{\catfont{Grp}}%{\calligra{Cat}}
\newcommand{\TWOCATS}{2\calligra{Cat}}%{\calligra{Cat}}
\newcommand{\OMEGACATS}{\omega\calligra{Cat}}%{\calligra{Cat}}
\newcommand{\TWOGROUPOIDS}{2\calligra{Gr}}%{\calligra{Cat}}
\newcommand{\OMEGAGROUPOIDS}{\omega\calligra{Gr}}%{\calligra{Cat}}
\newcommand{\DICATS}{\CATS_{\circlearrowright}}
\newcommand{\SITE}{\mathscr{X}}
\newcommand{\indexcat}[1]{{\ifthenelse{1=#1}{\mathscr{G}}{{\ifthenelse{2=#1}{\mathscr{H}}{\mathscr{I}}}}}}
\newcommand{\BOX}{\square}
\newcommand{\DEL}{\Delta}
\newcommand{\MONOIDAL}{\mathscr{V}}
\newcommand{\MEDIALSEMIGROUPS}{\calligra{Med}}
\newcommand{\SEMIAB}{\mathscr{A}}
\newcommand{\SEMIGROUPS}{\calligra{Sem}}
\newcommand{\Sh}{\mathop{Sh}\;\!\!\!}
\newcommand{\sheafification}{\callrsfs{Sheaf}}
\newcommand{\kernel}{\mathop{ker}}
\newcommand{\rank}{\mathop{rank}}
\newcommand{\nullity}{\mathop{null}}
\newcommand{\quotient}[2]{{\raisebox{.2em}{$#1$}\left/\raisebox{-.2em}{$#2$}\right.}}
\newcommand{\PRESHEAVES}[1]{\hat{#1}}
\newcommand{\MULTIPOINTED}[1]{{#1}_{\star\cdots\star}}
\newcommand{\TOPLATTICES}{\mathscr{K}}
\newcommand{\QUASIUNIFORM}{\mathscr{Q}}
\newcommand{\UNIFORM}{\mathscr{U}}
\newcommand{\BANACH}{\mathscr{B}}
\newcommand{\MODULES}{\mathscr{M}}
\newcommand{\COALGEBRAS}{\mathrm{Coalg}}
\newcommand{\HOMOTOPY}{h}
\newcommand{\Ch}{\mathop{Ch}\;\!\!}
\newcommand{\SEMICHAINS}{\mathop{ch}\;\!\!}

\newcommand{\SPACES}{\calligra{Top}}
\newcommand{\STREAMS}{\calligra{Str}}
\newcommand{\SETS}{\catfont{Set}}
\newcommand{\RELATIONS}{\calligra{Rel}}

% arithmetic
\newcommand{\half}{\nicefrac{1}{2}}
\newcommand{\third}{\nicefrac{1}{3}}
\newcommand{\fourth}{\nicefrac{1}{4}}
\newcommand{\fifth}{\nicefrac{1}{5}}
\newcommand{\sixth}{\nicefrac{1}{6}}
\newcommand{\seventh}{\nicefrac{1}{7}}
\newcommand{\eight}{\nicefrac{1}{8}}
\newcommand{\ninth}{\nicefrac{1}{9}}
\newcommand{\sign}[1]{\calligra{sign}(#1)}
\newcommand{\notdivides}{\nmid}
\newcommand{\divides}{\mid}


% algebra
\newcommand{\threebythree}[9]{\left(\begin{tabular}{ccc}#1&#2&#3\\#4&#5&#6\\#7&#8&#9\end{tabular}\right)}  
\newcommand{\twobythree}[6]{\left(\begin{tabular}{ccc}#1&#2&#3\\#4&#5&#6\end{tabular}\right)}  
\newcommand{\threebytwo}[6]{\left(\begin{tabular}{cc}#1&#2\\#3&#4\\#5&#6\end{tabular}\right)}  
\newcommand{\twobytwo}[4]{\left(\begin{tabular}{cc}#1&#2\\#3&#4\end{tabular}\right)}  
\newcommand{\semidirectproduct}{\rtimes}
\newcommand{\conjugate}[2]{\;\!^{#2}\!#1}
\newcommand{\ZPLUS}{\Z^+}
\newcommand{\ring}[1]{{\ifthenelse{1=#1}{R}{{\ifthenelse{2=#1}{S}{T}}}}}
\newcommand{\semiring}[1]{{\ifthenelse{0=#1}{\N}{{\ifthenelse{1=#1}{S}{T}}}}}
\newcommand{\semimodule}[1]{{\ifthenelse{1=#1}{M}{N}}}
\newcommand{\bitensor}[2]{\;\!\!_{#1}\otimes_{#2}}
\newcommand{\graded}[1]{{#1}_*}
\newcommand{\reversegraded}[1]{{#1}_{-*}}
\newcommand{\coreversegraded}[1]{{#1}^{-*}}
\newcommand{\leftshiftgraded}[2]{{#1}_{*-#2}}
\newcommand{\leftshiftreversegraded}[2]{{#1}_{#2-*}}
\newcommand{\rightshiftgraded}[2]{{#1}_{*+#2}}
\newcommand{\cograded}[1]{{#1}^*}
\newcommand{\dual}{{*}}
\newcommand{\groupcompletion}[1]{#1\otimes_{\N}\Z}
\newcommand{\grading}{{*}}
\newcommand{\tensor}[1]{{\ifthenelse{0=#1}{\otimes_\N\;}{{\ifthenelse{1=#1}{\otimes_{\semiring{1}}\;}{\otimes_{\semiring{1}[\Sigma_p]}}}}}}

% topology
\newcommand{\rel}[1]{\;\mathop{rel}\;#1}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\site}{\mathscr{O}}
\newcommand{\homotopic}{\sim}
\newcommand{\torus}{\T}
\newcommand{\interior}{\mathop{int}}
\newcommand{\topology}[1]{\mathscr{O}_{#1}}
\newcommand{\BASIS}{\mathscr{B}}
\newcommand{\deRham}{\Omega_{\mathrm{DR}}}
\newcommand{\der}[2]{\partial_{#1}^{#2}}
\newcommand{\loopspace}{\Omega}
\newcommand{\vectorfields}[1]{\mathfrak{X}(#1)}
\newcommand{\compactification}[1]{\mathbb{S}^{#1}}
\newcommand{\homology}[3]{\!\!\;_{#3}H^{#1}_{#2}}
\newcommand{\cohomology}[3]{\!\!\;_{#3}H_{#1}^{#2}}
\newcommand{\horn}[1]{\Lambda^{#1}}
\newcommand{\boxhorn}[1]{\sqcup^{#1}}
\newcommand{\eilenbergmaclane}[2]{K(#1,#2)}
\newcommand{\cycles}[1]{Z_{#1}}
\newcommand{\cocycles}[1]{Z^{#1}}
\newcommand{\fibrantreplacement}{R}
\newcommand{\fibrantextension}{\eta}  
\newcommand{\nerve}{\mathfrak{ner}}
\newcommand{\manifold}{M}
\newcommand{\leftderived}{L}
\newcommand{\rightderived}{R}
\newcommand{\filter}[1]{{\ifthenelse{1=#1}{\mathcal{F}}{{\ifthenelse{2=#1}{\mathcal{G}}{\mathcal{H}}}}}}

% geometry
\newcommand{\transport}{\nabla}

% ditopology
\newcommand{\disphere}[2]{\mathbb{S}^{#1,#2}}
\newcommand{\dihomotopic}{\leftrightsquigarrow}
\newcommand{\direalize}[1]{\upharpoonleft\!\!{#1}\!\!\downharpoonright}
\newcommand{\realize}[1]{|{#1}|}
\newcommand{\DI}[2]{\mathbb{I}^{(#1,#2)}}
\newcommand{\DS}[2]{\mathbb{S}^{(#1,#2)}}
\newcommand{\DR}[2]{\mathbb{R}^{(#1,#2)}}
\newcommand{\quasiuniformity}[1]{\ifthenelse{1=#1}{\mathscr{U}}{\ifthenelse{2=#1}{\mathscr{V}}{\mathscr{W}}}}

% order theory
\newcommand{\graph}{\mathop{graph}}
\newcommand{\meet}{\wedge}
\newcommand{\join}{\vee}

% simplicial and cubical sets
\newcommand{\Star}{\mathrm{Star}}
\newcommand{\openstar}{\mathrm{star}}
\newcommand{\sing}{\mathfrak{sing}}
\newcommand{\cosimplicial}{\nabla}
\newcommand{\tri}{\mathfrak{tri}\;\!\!}
\newcommand{\qua}{\mathfrak{qua}\;\!\!}
\newcommand{\sd}{\mathfrak{sd}}
\newcommand{\tot}{\mathfrak{tot}\;\!\!}
\newcommand{\sk}{\mathfrak{sk}\;\!\!}
\newcommand{\codiscrete}{\mathfrak{codisc}\;\!\!}
\newcommand{\tr}{\mathfrak{tr}}
\newcommand{\digraph}[1]{\ifthenelse{1=#1}{G}{\ifthenelse{2=#1}{H}{I}}}
\newcommand{\boxobj}[1]{[1]^{#1}}
\newcommand{\multiboxobj}[2]{[#1]^{#2}}
\newcommand{\support}{\mathfrak{supp}}
\newcommand{\totalization}{\mathfrak{tot}}
\newcommand{\decalage}{\mathfrak{dec}}  
\newcommand{\codiagonal}{\mathfrak{codiag}}  

% sheaf theory
\newcommand{\orientation}{\mathcal{O}}
\newcommand{\homsheaf}{\mathit{Hom}}
\newcommand{\constantsheaf}[1]{k_{#1}}
\newcommand{\constantcosheaf}[1]{k^{#1}}
\newcommand{\globalsections}{\Gamma}
\newcommand{\globalcosections}{\ensuremath{\reflectbox{$\Gamma$}}}
\newcommand{\sheaf}[1]{\ifthenelse{1=#1}{\mathcal{F}}{\ifthenelse{2=#1}{\mathcal{G}}{\mathcal{H}}}}
\newcommand{\connection}[1]{\ifthenelse{1=#1}{\nabla}{\ifthenelse{2=#1}{\nabla}{\nabla}}}
\newcommand{\structurecosheaf}{\mathcal{T}}
\newcommand{\cosheaf}[1]{\ifthenelse{1=#1}{\mathcal{X}}{\ifthenelse{2=#1}{\mathcal{Y}}{\mathcal{Z}}}}
\newcommand{\homologysheaf}{\mathcal{H}}

